Search for proton decay via $p\rightarrow{e^+\eta}$ and $p\rightarrow{\mu^+\eta}$ with a 0.37 Mton-year exposure of Super-Kamiokande

A search for proton decay into $e^+/\mu^+$ and a $\eta$ meson has been performed using data from a 0.373 Mton$\cdot$year exposure (6050.3 live days) of Super-Kamiokande. Compared to previous searches this work introduces an improved model of the intranuclear $\eta$ interaction cross section, resulting in a factor of two reduction in uncertainties from this source and $\sim$10\% increase in signal efficiency. No significant data excess was found above the expected number of atmospheric neutrino background events resulting in no indication of proton decay into either mode. Lower limits on the proton partial lifetime of $1.4\times\mathrm{10^{34}~years}$ for $p\rightarrow e^+\eta$ and $7.3\times\mathrm{10^{33}~years}$ for $p\rightarrow \mu^+\eta$ at the 90$\%$ C.L. were set. These limits are around 1.5 times longer than our previous study and are the most stringent to date.

==> SK-paper-acknowledgements-231213.tex <==
%Paper Acknowledgements(as of Dec. 1, 2023)


%Short list (in case number of lines are limited in short letter papers)

We gratefully acknowledge cooperation of the Kamioka Mining and Smelting Company.
The Super-Kamiokande experiment was built and has been operated with funding from the
Japanese Ministry of Education, Science, Sports and Culture, 
and the U.S. Department of Energy.



%Full list (for full papers and longer papers)

We gratefully acknowledge the cooperation of the Kamioka Mining and Smelting Company.
The Super-Kamiokande experiment has been built and operated from funding by the 
Japanese Ministry of Education, Culture, Sports, Science and Technology; the U.S.
Department of Energy; and the U.S. National Science Foundation. Some of us have been 
supported by funds from the National Research Foundation of Korea (NRF-2009-0083526 
and NRF 2022R1A5A1030700) funded by the Ministry of Science, 
Information and Communication Technology (ICT); the Institute for 
Basic Science (IBS-R016-Y2); and the Ministry of Education (2018R1D1A1B07049158,
2021R1I1A1A01042256, 2021R1I1A1A01059559); the Japan Society for the Promotion of Science; the National
Natural Science Foundation of China under Grants No.11620101004; the Spanish Ministry of Science, 
Universities and Innovation (grant PID2021-124050NB-C31); the Natural Sciences and 
Engineering Research Council (NSERC) of Canada; the Scinet and Westgrid consortia of
Compute Canada; 
the National Science Centre (UMO-2018/30/E/ST2/00441 and UMO-2022/46/E/ST2/00336) 
and the Ministry of Education and Science (2023/WK/04), Poland;
the Science and Technology Facilities Council (STFC) and
Grid for Particle Physics (GridPP), UK; the European Union's 
Horizon 2020 Research and Innovation Programme under the Marie Sklodowska-Curie grant
agreement no.754496; H2020-MSCA-RISE-2018 JENNIFER2 grant agreement no.822070, H2020-MSCA-RISE-2019 SK2HK grant agreement no. 872549; 
and European Union's Next Generation EU/PRTR  grant CA3/RSUE2021-00559.


